A Scalable Combinatorial Solver for Elastic Geometrically Consistent 3D Shape Matching

We present a scalable combinatorial algorithm for globally optimizing over the space of geometrically consistent mappings between 3D shapes. We use the mathematically elegant formalism proposed by Windheuser et al. (ICCV 2011) where 3D shape matching was formulated as an integer linear program over the space of orientation-preserving diffeomorphisms. Until now, the resulting formulation had limited practical applicability due to its complicated constraint structure and its large size. We propose a novel primal heuristic coupled with a Lagrange dual problem that is several orders of magnitudes faster compared to previous solvers. This allows us to handle shapes with substantially more triangles than previously solvable. We demonstrate compelling results on diverse datasets, and, even showcase that we can address the challenging setting of matching two partial shapes without availability of complete shapes. Our code is publicly available at http://github.com/paul0noah/sm-comb .

==> figures/pckKidsAll.tex <==
\begin{axis}[%
	legend columns=3,
	name=cat,
	width=\subplotwidth,
	height=\subplotheight,
	scale only axis,
	xmin=0,
	xmax=1,
	xtick={  0, 0.5,   1},
	ymin=0,
	ymax=103,
	ytick={  0,  50, 100},
	title={KIDS},
	axis x line*=bottom,
	axis y line*=left,
	legend style={legend cell align=left, align=left,
	legend to name=leg:sotaVsOurs2asdf,
	draw=white!15!black}
	]
\addplot [color=mycolor1, smooth, line width=\subplotlinewidth, forget plot]
  table[row sep=crcr]{%
0	5.46204620462046\\
0.01	9.00990099009901\\
0.02	19.7194719471947\\
0.03	30.5280528052805\\
0.04	39.3564356435644\\
0.05	46.8811881188119\\
0.06	53.019801980198\\
0.07	57.3597359735974\\
0.08	61.1056105610561\\
0.09	63.9273927392739\\
0.1	66.0891089108911\\
0.11	67.8877887788779\\
0.12	69.7524752475247\\
0.13	71.2211221122112\\
0.14	72.7722772277228\\
0.15	74.1089108910891\\
0.16	75.2970297029703\\
0.17	76.5841584158416\\
0.18	77.3927392739274\\
0.19	78.5148514851485\\
0.2	79.2574257425743\\
0.21	79.983498349835\\
0.22	80.8910891089109\\
0.23	81.6996699669967\\
0.24	82.3102310231023\\
0.25	82.8382838283828\\
0.26	83.2343234323432\\
0.27	83.6303630363036\\
0.28	83.993399339934\\
0.29	84.2244224422442\\
0.3	84.5214521452145\\
0.31	84.8019801980198\\
0.32	85.0660066006601\\
0.33	85.3135313531353\\
0.34	85.6105610561056\\
0.35	85.7920792079208\\
0.36	86.2211221122112\\
0.37	86.5016501650165\\
0.38	86.9306930693069\\
0.39	87.2937293729373\\
0.4	87.5742574257426\\
0.41	87.9207920792079\\
0.42	88.2673267326733\\
0.43	88.7128712871287\\
0.44	89.1914191419142\\
0.45	89.5049504950495\\
0.46	89.9009900990099\\
0.47	90.1980198019802\\
0.48	90.5280528052805\\
0.49	90.957095709571\\
0.5	91.2871287128713\\
0.51	91.6006600660066\\
0.52	92.0627062706271\\
0.53	92.5082508250825\\
0.54	92.8052805280528\\
0.55	93.1848184818482\\
0.56	93.4983498349835\\
0.57	93.6798679867987\\
0.58	93.8118811881188\\
0.59	93.976897689769\\
0.6	94.3399339933993\\
0.61	94.6039603960396\\
0.62	94.7854785478548\\
0.63	95\\
0.64	95.2805280528053\\
0.65	95.4620462046205\\
0.66	95.7425742574257\\
0.67	96.006600660066\\
0.68	96.2376237623762\\
0.69	96.5016501650165\\
0.7	96.7821782178218\\
0.71	96.947194719472\\
0.72	97.1947194719472\\
0.73	97.3762376237624\\
0.74	97.6567656765677\\
0.75	97.8712871287129\\
0.76	98.0858085808581\\
0.77	98.3333333333333\\
0.78	98.5973597359736\\
0.79	98.8613861386139\\
0.8	99.026402640264\\
0.81	99.2409240924092\\
0.82	99.3564356435644\\
0.83	99.5049504950495\\
0.84	99.5709570957096\\
0.85	99.5709570957096\\
0.86	99.7029702970297\\
0.87	99.7689768976898\\
0.88	99.8514851485149\\
0.89	99.8679867986799\\
0.9	99.8844884488449\\
0.91	99.8844884488449\\
0.92	99.9009900990099\\
0.93	99.96699669967\\
0.94	99.983498349835\\
0.95	99.983498349835\\
0.96	99.983498349835\\
0.97	99.983498349835\\
0.98	100\\
1	100\\
};

\addplot [color=mycolor2, smooth, line width=\subplotlinewidth, forget plot]
  table[row sep=crcr]{%
0	2.88778877887789\\
0.01	4.43894389438944\\
0.02	9.93399339933993\\
0.03	15.6930693069307\\
0.04	21.4356435643564\\
0.05	26.6171617161716\\
0.06	31.0561056105611\\
0.07	34.8184818481848\\
0.08	38.0858085808581\\
0.09	40.6765676567657\\
0.1	42.9372937293729\\
0.11	44.7029702970297\\
0.12	46.2211221122112\\
0.13	47.3927392739274\\
0.14	48.8778877887789\\
0.15	50\\
0.16	51.006600660066\\
0.17	52.046204620462\\
0.18	53.2013201320132\\
0.19	54.4884488448845\\
0.2	55.6105610561056\\
0.21	56.947194719472\\
0.22	58.3828382838284\\
0.23	59.7524752475247\\
0.24	60.8580858085809\\
0.25	61.8976897689769\\
0.26	62.8217821782178\\
0.27	63.8283828382838\\
0.28	64.9009900990099\\
0.29	65.9405940594059\\
0.3	66.8976897689769\\
0.31	67.7722772277228\\
0.32	68.7458745874587\\
0.33	69.7524752475247\\
0.34	70.6270627062706\\
0.35	71.6666666666667\\
0.36	72.6402640264026\\
0.37	73.3168316831683\\
0.38	74.0594059405941\\
0.39	74.7854785478548\\
0.4	75.5610561056106\\
0.41	76.6336633663366\\
0.42	77.4257425742574\\
0.43	78.2673267326733\\
0.44	79.026402640264\\
0.45	79.6864686468647\\
0.46	80.4125412541254\\
0.47	80.973597359736\\
0.48	81.6501650165016\\
0.49	82.1122112211221\\
0.5	82.5412541254126\\
0.51	83.1188118811881\\
0.52	83.6798679867987\\
0.53	84.1914191419142\\
0.54	84.5544554455445\\
0.55	84.8679867986799\\
0.56	85.2805280528053\\
0.57	85.9075907590759\\
0.58	86.3366336633663\\
0.59	86.8976897689769\\
0.6	87.4422442244224\\
0.61	88.019801980198\\
0.62	88.4983498349835\\
0.63	88.943894389439\\
0.64	89.3399339933993\\
0.65	90.0660066006601\\
0.66	90.6270627062706\\
0.67	91.1386138613861\\
0.68	91.5016501650165\\
0.69	91.9306930693069\\
0.7	92.3432343234323\\
0.71	92.7722772277228\\
0.72	93.1848184818482\\
0.73	93.5643564356436\\
0.74	93.993399339934\\
0.75	94.4554455445545\\
0.76	94.8019801980198\\
0.77	95.1650165016502\\
0.78	95.5940594059406\\
0.79	96.1386138613861\\
0.8	96.6666666666667\\
0.81	97.1122112211221\\
0.82	97.3102310231023\\
0.83	97.5907590759076\\
0.84	97.8547854785479\\
0.85	98.036303630363\\
0.86	98.2013201320132\\
0.87	98.3498349834984\\
0.88	98.4818481848185\\
0.89	98.6138613861386\\
0.9	98.8283828382838\\
0.91	99.0594059405941\\
0.92	99.2739273927393\\
0.93	99.3894389438944\\
0.94	99.5544554455445\\
0.95	99.7194719471947\\
0.96	99.7854785478548\\
0.97	99.9174917491749\\
0.98	99.96699669967\\
1	100\\
};

\addplot [color=mycolor3, smooth, line width=\subplotlinewidth, forget plot]
  table[row sep=crcr]{%
0	6.72613148331681\\
0.01	10.8820614469772\\
0.02	24.3145028080608\\
0.03	38.3019491245458\\
0.04	50.0561612157251\\
0.05	59.7092831185993\\
0.06	67.6511397423191\\
0.07	73.7628014535844\\
0.08	78.5992732077965\\
0.09	82.5371655104063\\
0.1	85.1668318467129\\
0.11	87.1423851998679\\
0.12	88.8999008919723\\
0.13	90.1552692434754\\
0.14	90.796167822927\\
0.15	91.3247439709283\\
0.16	91.6617112652792\\
0.17	91.9590353485299\\
0.18	92.2629666336307\\
0.19	92.6329699372316\\
0.2	92.778328377932\\
0.21	92.9501156260324\\
0.22	93.1152956722828\\
0.23	93.2738685166832\\
0.24	93.4522629666336\\
0.25	93.584407003634\\
0.26	93.7363726461843\\
0.27	93.9081598942848\\
0.28	93.9610175090849\\
0.29	94.0997687479353\\
0.3	94.3376280145359\\
0.31	94.4895936570862\\
0.32	94.7340601255368\\
0.33	95.1106706309878\\
0.34	95.2692434753882\\
0.35	95.3881731086885\\
0.36	95.6656755863892\\
0.37	95.7515692104394\\
0.38	95.9497852659399\\
0.39	96.1017509084903\\
0.4	96.1744301288404\\
0.41	96.3528245787909\\
0.42	96.4387182028411\\
0.43	96.5840766435415\\
0.44	96.7096134786918\\
0.45	96.8615791212422\\
0.46	97.0862239841427\\
0.47	97.198546415593\\
0.48	97.3306904525933\\
0.49	97.4694416914437\\
0.5	97.614800132144\\
0.51	97.6808721506442\\
0.52	97.8394449950446\\
0.53	97.8592666005947\\
0.54	97.8592666005947\\
0.55	97.8989098116948\\
0.56	97.991410637595\\
0.57	98.1565906838454\\
0.58	98.2226627023456\\
0.59	98.3217707300958\\
0.6	98.4407003633961\\
0.61	98.5860588040965\\
0.62	98.7049884373968\\
0.63	98.797489263297\\
0.64	98.9296333002973\\
0.65	99.0023125206475\\
0.66	99.0485629335976\\
0.67	99.180706970598\\
0.68	99.200528576148\\
0.69	99.2467789890981\\
0.7	99.2930294020482\\
0.71	99.3789230260984\\
0.72	99.4317806408986\\
0.73	99.4846382556987\\
0.74	99.596960687149\\
0.75	99.7158903204493\\
0.76	99.7687479352494\\
0.77	99.8149983481995\\
0.78	99.8942847703997\\
0.79	99.9339279814998\\
0.8	99.9735711925999\\
0.81	100\\
0.82	100\\
0.83	100\\
0.84	100\\
0.85	100\\
0.86	100\\
0.87	100\\
0.88	100\\
0.89	100\\
0.9	100\\
0.91	100\\
0.92	100\\
0.93	100\\
0.94	100\\
0.95	100\\
0.96	100\\
0.97	100\\
0.98	100\\
1	100\\
};
\end{axis}

==> figures/pckShrec19all.tex <==
\begin{axis}[%
	legend columns=3,
	name=cat,
	width=\subplotwidth,
	height=\subplotheight,
	scale only axis,
	xmin=0,
	xmax=1,
	xtick={  0, 0.5,   1},
	ymin=0,
	ymax=103,
	ytick={  0,  50, 100},
	title={SHREC'19},
	axis x line*=bottom,
	axis y line*=left,
	legend style={legend cell align=left, align=left,
	legend to name=leg:sotaVsOurs2,
	draw=white!15!black}
	]
\addplot [color=mycolor1, smooth, line width=\subplotlinewidth]
  table[row sep=crcr]{%
0	10.0344290663593\\
0.01	11.9937221218908\\
0.02	18.2453944170554\\
0.03	24.6453103902085\\
0.04	30.4461776683413\\
0.05	35.647077041492\\
0.06	39.8041449174146\\
0.07	43.3909882272026\\
0.08	46.4087901529888\\
0.09	48.9511412500564\\
0.1	51.1929297705462\\
0.11	53.3017003926378\\
0.12	55.2529224156093\\
0.13	56.9701199229044\\
0.14	58.537856931157\\
0.15	59.9605766765279\\
0.16	61.2860070935274\\
0.17	62.7286148204408\\
0.18	64.0813094433288\\
0.19	65.4526452022894\\
0.2	66.8797099972476\\
0.21	68.1298550212904\\
0.22	69.3959132982033\\
0.23	70.5597690613258\\
0.24	71.6806951222854\\
0.25	72.6233689359197\\
0.26	73.4816114310872\\
0.27	74.2552741114969\\
0.28	75.0051408242299\\
0.29	75.6728421376911\\
0.3	76.3316790804718\\
0.31	76.8914524591149\\
0.32	77.4589086455627\\
0.33	78.0264142111238\\
0.34	78.5252698049433\\
0.35	79.0262606448561\\
0.36	79.612968492707\\
0.37	80.1973646436917\\
0.38	80.7481154949114\\
0.39	81.2457943336466\\
0.4	81.7828497051213\\
0.41	82.280500400812\\
0.42	82.8230998807941\\
0.43	83.3312041636124\\
0.44	83.8289620761752\\
0.45	84.3393093512992\\
0.46	84.8585646892215\\
0.47	85.3913597628446\\
0.48	85.8979856969425\\
0.49	86.353009688106\\
0.5	86.7516598644864\\
0.51	87.1279238650198\\
0.52	87.5222070332974\\
0.53	87.8681013221161\\
0.54	88.2399554925454\\
0.55	88.6136519217482\\
0.56	88.9899159222816\\
0.57	89.4101795221415\\
0.58	89.8214116338543\\
0.59	90.1943828109873\\
0.6	90.5842445826313\\
0.61	90.9684044525201\\
0.62	91.3761439548066\\
0.63	91.7635733310175\\
0.64	92.1364141536754\\
0.65	92.5339547460368\\
0.66	92.932720413916\\
0.67	93.372087201606\\
0.68	93.7562967868411\\
0.69	94.1629313692059\\
0.7	94.5357264408866\\
0.71	94.8948919929947\\
0.72	95.2271638214302\\
0.73	95.5796660205601\\
0.74	95.917532713354\\
0.75	96.2554581140237\\
0.76	96.5560942347592\\
0.77	96.8568774386986\\
0.78	97.1249493644102\\
0.79	97.3840262105587\\
0.8	97.6160622361997\\
0.81	97.8581609599072\\
0.82	98.048540352191\\
0.83	98.2400388231008\\
0.84	98.4292521703442\\
0.85	98.6117439906175\\
0.86	98.8055235935624\\
0.87	98.959859322314\\
0.88	99.075868183576\\
0.89	99.1918870596975\\
0.9	99.2809146784442\\
0.91	99.3473984984847\\
0.92	99.4048887997192\\
0.93	99.4623690860941\\
0.94	99.5186930060554\\
0.95	99.5705200791476\\
0.96	99.6133436185742\\
0.97	99.6437540894554\\
0.98	99.6584008215441\\
1	99.6628976684132\\
};
\addlegendentry{\textcolor{black}{Eisenb.'20}}

\addplot [color=mycolor2, smooth, line width=\subplotlinewidth]
  table[row sep=crcr]{%
0	9.47264114020358\\
0.01	11.2148268023328\\
0.02	16.863410319931\\
0.03	23.0397804070799\\
0.04	29.18667953423\\
0.05	34.483898651893\\
0.06	39.2459360872584\\
0.07	42.9878447409453\\
0.08	46.1965338086458\\
0.09	48.831492273047\\
0.1	51.0412381379572\\
0.11	52.8934549184531\\
0.12	54.5679424626554\\
0.13	56.0719368831456\\
0.14	57.4350160069309\\
0.15	58.7305304257352\\
0.16	59.9448441974808\\
0.17	61.2581786795568\\
0.18	62.5084665083518\\
0.19	63.7170377895643\\
0.2	65.0024636095685\\
0.21	66.1919424357131\\
0.22	67.3922754947679\\
0.23	68.485818539175\\
0.24	69.4892071182041\\
0.25	70.3829350909003\\
0.26	71.2022688747196\\
0.27	71.9342419351543\\
0.28	72.6577321565254\\
0.29	73.3057710783663\\
0.3	73.9334820776358\\
0.31	74.535160862598\\
0.32	75.1213020839743\\
0.33	75.7230502823126\\
0.34	76.3369757135384\\
0.35	76.9163871287741\\
0.36	77.5745683654802\\
0.37	78.2486105475351\\
0.38	78.9303362189483\\
0.39	79.5726946727531\\
0.4	80.2309230326306\\
0.41	80.8463977867099\\
0.42	81.3771330176182\\
0.43	81.8991009094706\\
0.44	82.4336106772173\\
0.45	82.9622690427623\\
0.46	83.4853729396199\\
0.47	84.0347236730927\\
0.48	84.5544478956297\\
0.49	84.9169572246397\\
0.5	85.2803295965102\\
0.51	85.6404490294865\\
0.52	85.93961888374\\
0.53	86.2194115747758\\
0.54	86.4992311934191\\
0.55	86.7881410353475\\
0.56	87.0692050776744\\
0.57	87.3785446764784\\
0.58	87.7037648868552\\
0.59	88.086604210359\\
0.6	88.455971821169\\
0.61	88.8556611549494\\
0.62	89.3061358167907\\
0.63	89.7610779624759\\
0.64	90.2609699284138\\
0.65	90.7531525133471\\
0.66	91.2824867714431\\
0.67	91.8310226121007\\
0.68	92.3704770561581\\
0.69	92.8988712740319\\
0.7	93.4058188451159\\
0.71	93.9216801705374\\
0.72	94.4455868657609\\
0.73	94.9175672048696\\
0.74	95.3276702140094\\
0.75	95.7285820129581\\
0.76	96.09808409085\\
0.77	96.4550549983481\\
0.78	96.8189238790453\\
0.79	97.1311043384705\\
0.8	97.4206512198612\\
0.81	97.7495228421793\\
0.82	97.9668627566184\\
0.83	98.2088428673122\\
0.84	98.40820524329\\
0.85	98.5714845960256\\
0.86	98.7660276089443\\
0.87	98.9578882405868\\
0.88	99.0815781739642\\
0.89	99.1682928758642\\
0.9	99.2437306800686\\
0.91	99.2944112266746\\
0.92	99.3338250562893\\
0.93	99.3721122142048\\
0.94	99.4002396469732\\
0.95	99.4362734614905\\
0.96	99.4678104291387\\
0.97	99.5106042738508\\
0.98	99.5207344792155\\
1	99.5207344792155\\
};
\addlegendentry{\textcolor{black}{Ren '21}}

\addplot [color=mycolor3, smooth, line width=\subplotlinewidth]
  table[row sep=crcr]{%
0	12.3454456689814\\
0.01	15.6340184775034\\
0.02	26.2655981393207\\
0.03	37.0786053253508\\
0.04	47.1566142586911\\
0.05	55.9786584209882\\
0.06	62.9124459674616\\
0.07	68.1596049881774\\
0.08	71.7700291404282\\
0.09	74.4762911409901\\
0.1	76.4111604440488\\
0.11	77.9502822508793\\
0.12	79.1410489199696\\
0.13	80.1822249358002\\
0.14	80.981027614947\\
0.15	81.6503726017743\\
0.16	82.3276589365919\\
0.17	83.0772026006767\\
0.18	83.7801308326977\\
0.19	84.6575445277371\\
0.2	85.4106763721528\\
0.21	86.0794331851332\\
0.22	86.8200186450804\\
0.23	87.4217121969121\\
0.24	87.9948254978037\\
0.25	88.5348924670548\\
0.26	89.0491174370273\\
0.27	89.4422987502399\\
0.28	89.8908625130159\\
0.29	90.2549829967972\\
0.3	90.6014375681503\\
0.31	90.9562332350984\\
0.32	91.2760220392798\\
0.33	91.5764003201848\\
0.34	91.8809572354767\\
0.35	92.1542501414112\\
0.36	92.3995717093216\\
0.37	92.6459222251419\\
0.38	92.9593090840628\\
0.39	93.2120151507726\\
0.4	93.4364142668083\\
0.41	93.688857828642\\
0.42	93.9626483330634\\
0.43	94.1913733382365\\
0.44	94.3869550855042\\
0.45	94.6320830572223\\
0.46	94.8101852083289\\
0.47	95.0593677668341\\
0.48	95.2197878821477\\
0.49	95.3612383001687\\
0.5	95.4883803050491\\
0.51	95.6335560970251\\
0.52	95.785141292698\\
0.53	95.9143380590738\\
0.54	96.0788818321161\\
0.55	96.2144503241684\\
0.56	96.3523298575503\\
0.57	96.4789228672385\\
0.58	96.6636588201274\\
0.59	96.7930386223083\\
0.6	96.9272899213924\\
0.61	97.0356195549452\\
0.62	97.1835987111507\\
0.63	97.326796609303\\
0.64	97.4519348514005\\
0.65	97.6104500535948\\
0.66	97.7718731551677\\
0.67	97.8901358356802\\
0.68	98.0119903067475\\
0.69	98.1759669029373\\
0.7	98.3085487144151\\
0.71	98.4369244172952\\
0.72	98.5600440511087\\
0.73	98.6581498774979\\
0.74	98.7971641337497\\
0.75	98.8847628643069\\
0.76	99.0039596333669\\
0.77	99.1327940201238\\
0.78	99.2146163772203\\
0.79	99.2826087375498\\
0.8	99.3579288453461\\
0.81	99.4548427726765\\
0.82	99.5383292176884\\
0.83	99.6084981461711\\
0.84	99.66309382637\\
0.85	99.7126707913269\\
0.86	99.7519592981824\\
0.87	99.7829331573038\\
0.88	99.7986626976062\\
0.89	99.8108279820175\\
0.9	99.8204326657405\\
0.91	99.8221292548368\\
0.92	99.8225512919254\\
0.93	99.8292613059338\\
0.94	99.8308642954692\\
0.95	99.8312437531483\\
0.96	99.8332687797723\\
0.97	99.8349569281268\\
0.98	99.8365173382526\\
1	99.8365173382526\\
};
\addlegendentry{\textcolor{black}{Ours}}
\end{axis}

==> figures/pckToscaAll.tex <==
\begin{axis}[%
	legend columns=3,
	name=cat,
	width=\subplotwidth,
	height=\subplotheight,
	scale only axis,
	xmin=0,
	xmax=1,
	xtick={  0, 0.5,   1},
	ymin=0,
	ymax=103,
	ytick={  0,  50, 100},
	title={TOSCA},
	axis x line*=bottom,
	axis y line*=left,
	legend style={legend cell align=left, align=left,
	legend to name=leg:pckCombinedLeg,
	draw=white!15!black}
	]
    \addplot [color=mycolor1, smooth, line width=\subplotlinewidth]
      table[row sep=crcr]{%
        0	12.9374879485012\\
        0.01	20.1728741156054\\
        0.02	36.4766608819472\\
        0.03	49.8454812441597\\
        0.04	59.7265978433379\\
        0.05	66.6798306115487\\
        0.06	71.4688366780878\\
        0.07	74.8637995223898\\
        0.08	77.2386122606387\\
        0.09	79.037660006823\\
        0.1	80.5854803542028\\
        0.11	81.9340245331435\\
        0.12	83.0582625076017\\
        0.13	83.9369465580919\\
        0.14	84.7534077930554\\
        0.15	85.6337605126151\\
        0.16	86.3874056274937\\
        0.17	86.9732938785802\\
        0.18	87.4682582061437\\
        0.19	88.0157670686305\\
        0.2	88.4814369836396\\
        0.21	88.8859965291683\\
        0.22	89.2845117845118\\
        0.23	89.6268114329789\\
        0.24	89.8997315296875\\
        0.25	90.1778059597443\\
        0.26	90.4278096678978\\
        0.27	90.7035108797223\\
        0.28	90.8876948634658\\
        0.29	91.1261662142719\\
        0.3	91.3803601358667\\
        0.31	91.6078924338836\\
        0.32	91.8220012162743\\
        0.33	92.0473457037334\\
        0.34	92.2842225485397\\
        0.35	92.5036339904181\\
        0.36	92.691674453789\\
        0.37	92.9071181714353\\
        0.38	93.1887895103754\\
        0.39	93.3878061080704\\
        0.4	93.6595766771978\\
        0.41	93.8131313131313\\
        0.42	94.0404040404041\\
        0.43	94.1989646835462\\
        0.44	94.4006882332874\\
        0.45	94.6089752147021\\
        0.46	94.7802177427728\\
        0.47	95.0005933045581\\
        0.48	95.2486687728979\\
        0.49	95.4621471691956\\
        0.5	95.7775997864104\\
        0.51	96.0014239309393\\
        0.52	96.2409335647221\\
        0.53	96.4296044141859\\
        0.54	96.6020706329076\\
        0.55	96.778615820466\\
        0.56	96.9747400584405\\
        0.57	97.2329017042673\\
        0.58	97.3629837286225\\
        0.59	97.5717156884558\\
        0.6	97.8028819768908\\
        0.61	97.9777584953796\\
        0.62	98.1162951096872\\
        0.63	98.2427060620893\\
        0.64	98.3899197555585\\
        0.65	98.5171094201931\\
        0.66	98.5815200462778\\
        0.67	98.6406650944096\\
        0.68	98.6981785550067\\
        0.69	98.7720078909506\\
        0.7	98.8282976608968\\
        0.71	98.8939690591673\\
        0.72	98.9453640665094\\
        0.73	99.0215666206855\\
        0.74	99.0851985345377\\
        0.75	99.120648481882\\
        0.76	99.2030436523829\\
        0.77	99.244649134517\\
        0.78	99.2768359067919\\
        0.79	99.328230914134\\
        0.8	99.3755469526395\\
        0.81	99.4554947418384\\
        0.82	99.556949821267\\
        0.83	99.6588498791142\\
        0.84	99.713730550735\\
        0.85	99.7511829009626\\
        0.86	99.807398507839\\
        0.87	99.8448508580667\\
        0.88	99.8823773713642\\
        0.89	99.9015114433617\\
        0.9	99.912116762337\\
        0.91	99.914564143639\\
        0.92	99.9186431124757\\
        0.93	99.9344398463341\\
        0.94	99.9462317744256\\
        0.95	99.9621026713538\\
        0.96	99.98776309349\\
        0.97	100\\
        0.98	100\\
        1	100\\
    };
    \addlegendentry{{\textcolor{black}{Eisenberger et al. '20}}}
    
    \addplot [color=mycolor2, smooth, line width=\subplotlinewidth]
      table[row sep=crcr]{%
        0	6.79574748958009\\
        0.01	10.20361470802\\
        0.02	18.5296429789822\\
        0.03	26.8777347631973\\
        0.04	34.3701330485471\\
        0.05	40.6384327860099\\
        0.06	45.7345110428811\\
        0.07	49.6696776872988\\
        0.08	52.65155223305\\
        0.09	55.0316676307866\\
        0.1	57.0057402215993\\
        0.11	58.7938118334594\\
        0.12	60.5326762485353\\
        0.13	62.424687402661\\
        0.14	64.1510553404827\\
        0.15	65.9371987125291\\
        0.16	67.5518770672956\\
        0.17	69.1328112253222\\
        0.18	70.6825598125157\\
        0.19	72.2655705364956\\
        0.2	73.7618846319287\\
        0.21	75.0337812782747\\
        0.22	76.375094557914\\
        0.23	77.4339577863807\\
        0.24	78.4015633575105\\
        0.25	79.4097361277978\\
        0.26	80.2774440439639\\
        0.27	80.7815304291075\\
        0.28	81.4160696539551\\
        0.29	81.9945045165309\\
        0.3	82.5566976668298\\
        0.31	82.993888963052\\
        0.32	83.3636289473294\\
        0.33	83.7932926919711\\
        0.34	84.2914460315341\\
        0.35	84.7049051454338\\
        0.36	85.1415402186327\\
        0.37	85.6384698675448\\
        0.38	86.3134650469452\\
        0.39	86.8124712618105\\
        0.4	87.282924694819\\
        0.41	87.7434773580148\\
        0.42	88.1764413592607\\
        0.43	88.6239413221792\\
        0.44	89.1009952683962\\
        0.45	89.4489683916997\\
        0.46	89.775248817099\\
        0.47	90.0626677939453\\
        0.48	90.4348922410597\\
        0.49	90.7565374745991\\
        0.5	91.0598273483736\\
        0.51	91.4121760927928\\
        0.52	91.8400599237604\\
        0.53	92.3103279490945\\
        0.54	92.6488823625387\\
        0.55	92.9213574808289\\
        0.56	93.228095937347\\
        0.57	93.3937020721162\\
        0.58	93.6217164300865\\
        0.59	93.946402349486\\
        0.6	94.2910752161854\\
        0.61	94.5439712840594\\
        0.62	94.7760646108664\\
        0.63	95.0411975852504\\
        0.64	95.2325012236906\\
        0.65	95.4352259748736\\
        0.66	95.6787404144232\\
        0.67	95.9132811225322\\
        0.68	96.1306901615272\\
        0.69	96.4582313591124\\
        0.7	96.6332191222059\\
        0.71	96.8649045521292\\
        0.72	97.021129058574\\
        0.73	97.277696198401\\
        0.74	97.511013215859\\
        0.75	97.6741719693262\\
        0.76	97.8250938162832\\
        0.77	98.0282264643498\\
        0.78	98.1175558818731\\
        0.79	98.2370696687877\\
        0.8	98.3231359112416\\
        0.81	98.4169521944852\\
        0.82	98.552373959863\\
        0.83	98.672703540545\\
        0.84	98.8191385217817\\
        0.85	99.0899820525371\\
        0.86	99.2723119595366\\
        0.87	99.4925762767173\\
        0.88	99.5978136727036\\
        0.89	99.7071300375265\\
        0.9	99.8070647740251\\
        0.91	99.8445912873226\\
        0.92	99.9090389949421\\
        0.93	99.9449339207048\\
        0.94	99.9665524555392\\
        0.95	99.986539402839\\
        0.96	99.991434165443\\
        0.97	100\\
        0.98	100\\
        1	100\\
    };
    \addlegendentry{{\textcolor{black}{Ren et al. '21}}}
    
    \addplot [color=mycolor3, smooth, line width=\subplotlinewidth]
      table[row sep=crcr]{%
        0	12.0276332036509\\
        0.01	19.2692543465284\\
        0.02	36.0612853529347\\
        0.03	49.5851507004897\\
        0.04	61.4684513051172\\
        0.05	70.3791462230181\\
        0.06	76.5304418408078\\
        0.07	81.0058957819065\\
        0.08	84.3156840286285\\
        0.09	86.2714307091168\\
        0.1	87.7802275837087\\
        0.11	89.0203109098328\\
        0.12	89.8312816168035\\
        0.13	90.3817747544876\\
        0.14	90.8918281093705\\
        0.15	91.2130580946054\\
        0.16	91.4422403891346\\
        0.17	91.8000718687634\\
        0.18	92.1560996263337\\
        0.19	92.4612300053745\\
        0.2	92.7249574501891\\
        0.21	92.949342915708\\
        0.22	93.1866624217389\\
        0.23	93.301569604041\\
        0.24	93.5289571980116\\
        0.25	93.6800475310005\\
        0.26	93.7801020047889\\
        0.27	93.9630368316619\\
        0.28	94.178193390657\\
        0.29	94.3375369016236\\
        0.3	94.5046297690912\\
        0.31	94.6665245120567\\
        0.32	94.7837192623073\\
        0.33	94.8868009609943\\
        0.34	94.977022648847\\
        0.35	95.1115439413641\\
        0.36	95.2950370944604\\
        0.37	95.5106115469797\\
        0.38	95.6317611378474\\
        0.39	95.8388120893554\\
        0.4	95.9766390852586\\
        0.41	96.0740434223911\\
        0.42	96.1938387248706\\
        0.43	96.4107480030268\\
        0.44	96.5170389588962\\
        0.45	96.7076272621615\\
        0.46	96.8284813454836\\
        0.47	96.9162376151747\\
        0.48	97.0167803365208\\
        0.49	97.1014291490714\\
        0.5	97.2300666467266\\
        0.51	97.353789621956\\
        0.52	97.5402375167341\\
        0.53	97.5954698928935\\
        0.54	97.6885482474936\\
        0.55	97.7415438377766\\
        0.56	97.8143489955538\\
        0.57	97.9374839855551\\
        0.58	97.9971127176125\\
        0.59	98.0403601431666\\
        0.6	98.1336221214072\\
        0.61	98.2484035540308\\
        0.62	98.3246627209395\\
        0.63	98.3411794471308\\
        0.64	98.3782306732512\\
        0.65	98.4277099579105\\
        0.66	98.5073535399111\\
        0.67	98.6594338611255\\
        0.68	98.6832871903474\\
        0.69	98.7159541462233\\
        0.7	98.7764210135572\\
        0.71	98.9492181176671\\
        0.72	99.0754198279565\\
        0.73	99.1117795372283\\
        0.74	99.2005025319541\\
        0.75	99.2321509205406\\
        0.76	99.2769979274926\\
        0.77	99.3079450910126\\
        0.78	99.3326134437065\\
        0.79	99.4012297921651\\
        0.8	99.4131846253891\\
        0.81	99.4768493912184\\
        0.82	99.5289040326295\\
        0.83	99.5697672250036\\
        0.84	99.5823984548033\\
        0.85	99.6506597854409\\
        0.86	99.6871301477958\\
        0.87	99.7641148579827\\
        0.88	99.7733757636251\\
        0.89	99.8476324256908\\
        0.9	99.9786244577911\\
        0.91	99.9786244577911\\
        0.92	99.9953078078078\\
        0.93	99.9953078078078\\
        0.94	99.9962462462462\\
        0.95	99.9962462462462\\
        0.96	100\\
        0.97	100\\
        0.98	100\\
        1	100\\
    };
    \addlegendentry{{\textcolor{black}{Ours}}}
    \end{axis}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
